On the Effective Use of Pretraining for Natural Language Inference

Neural networks have excelled at many NLP tasks, but there remain open questions about the performance of pretrained distributed word representations and their interaction with weight initialization and other hyperparameters. We address these questions empirically using attention-based sequence-to-sequence models for natural language inference (NLI). Specifically, we compare three types of embeddings: random, pretrained (GloVe, word2vec), and retrofitted (pretrained plus WordNet information). We show that pretrained embeddings outperform both random and retrofitted ones in a large NLI corpus. Further experiments on more controlled data sets shed light on the contexts for which retrofitted embeddings can be useful. We also explore two principled approaches to initializing the rest of the model parameters, Gaussian and orthogonal, showing that the latter yields gains of up to 2.9% in the NLI task.

==> embedding-classes.tex <==
\subsection{Embedding Classes}\label{sec:embedding-classes}

Our central hypothesis is that the structure of the inputs is an
important factor in task performance. To evaluate this idea, we test
random, GloVe \cite{pennington2014}, and word2vec
\cite{Mikolov-etal:2013:ICLR,Goldberg:Levy:2014} inputs, as well
variants of GloVe and word2vec that have been retrofitted with WordNet
information \cite{faruqui2014}.

For the definitions of the GloVe and word2vec models, we refer to the
original papers. We used the publicly released embeddings, trained with Common Crawl 840B tokens for GloVe and Google News 42B for word2vec. Although the training data sizes are notably different, our goal is not to compare these models directly, but with their retrofitted versions and random.

The further step of retrofitting is defined as
follows. Given a $d$-dimensional vector for a word $j$ drawn from a
vocabulary $V$, $\bm{x}_j$, is retrofitted into a vector
$\bm{\tilde{x}}_j$ by minimizing an objective that seeks to keep the
retrofitted vector $\bm{\tilde{x}}_j$ close to the original, but
changed in a way that incorporates a notion of distance defined by a
source external to the embedding space $E$, such as WordNet
\cite{WordNet98}.  The objective of \newcite{faruqui2014} is defined
as follows:
%
\begin{equation}
\sum_{j \in V} 
  \Bigg\{ 
    \alpha_j \norm{\bm{\tilde{x}}_j - \bm{x}_j}^2 + 
    \sum_{i,j \in E} \beta_{ij} \norm{\bm{\tilde{x}}_i - \bm{\tilde{x}}_j}^2 
  \Bigg\}
\end{equation}
%
In our experiments, we used the off-the-shelf algorithm provided by
the authors, keeping the pre-established parameters.

\subsection{Embedding Preprocessing}

GloVe and word2vec embeddings can generally be used directly, with no
preprocessing steps required. However, retrofitting pretrained
embeddings generates vectors that are not centered and with amplitudes
one magnitude lower than those of GloVe or word2vec. We therefore took
two simple preprocessing steps that helped performance.

First, each dimension was mean centered. This step makes the
distribution of inputs more similar to the distribution of weights,
which is especially important because of the coupling of inputs and
parameters discussed in Section~\ref{sec:motivation}.

Second, each embedding dimension was rescaled to have a standard
deviation of one.  Rescaling is usually applied to inputs showing high
variance for features that should contribute equally. As such, it has
only a small effect for embeddings in general because the amplitudes
are typically of the same order, and the impact of the amplitudes is
absorbed by adjusting the initialization range of the weight
distribution via hyper-parameter search.

The overall effect of these two preprocessing steps was to give all
our input vectors similar overall summary statistics.
